Rearrangement Planning for General Part Assembly

Most successes in autonomous robotic assembly have been restricted to single target or category. We propose to investigate general part assembly, the task of creating novel target assemblies with unseen part shapes. As a fundamental step to a general part assembly system, we tackle the task of determining the precise poses of the parts in the target assembly, which we we term ``rearrangement planning''. We present General Part Assembly Transformer (GPAT), a transformer-based model architecture that accurately predicts part poses by inferring how each part shape corresponds to the target shape. Our experiments on both 3D CAD models and real-world scans demonstrate GPAT's generalization abilities to novel and diverse target and part shapes.

==> tables/table_cat_swap.tex <==
\begin{table*}[th]
\vspace{-3mm}
\caption{To validate GPAT's dependence on the training dataset, we swap the training and testing categories and show the by category results in Table~\ref{table:swap}.} \label{table:swap}
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
& \multicolumn{6}{c}{Canonical Pose} & \multicolumn{6}{c}{Random Pose}  \\
& \multicolumn{3}{c|}{Precise Part} & \multicolumn{3}{c|}{Imprecise Part} & \multicolumn{3}{c|}{Precise Part} & \multicolumn{3}{c}{Imprecise Part}  \\ 
& CD & PA & SR & CD & PA & SR & CD & PA & SR & CD & PA & SR \\
\hline
Table  & 8.6 & 46.5 & 14.6 & 8.8 & 48.9 & 15.0 & 8.2 & 48.7 & 16.2 & 8.3 & 53.2 & 18.3 \\ 
Display  & 6.0 & 60.6 & 25.6 & 5.6 & 63.6 & 25.8 & 5.8 & 60.4 & 26.2 & 5.9 & 61.3 & 27.0 \\ 
\midrule
Chair  & 29.3 & 13.7 & 0.0 & 25.9 & 15.6 & 0.0 & 25.9 & 17.2 & 0.0 & 23.3 & 20.8 & 0.4 \\ 
Lamp  & 23.3 & 19.9 & 2.3 & 16.9 & 27.9 & 6.4 & 22.8 & 20.9 & 3.1 & 19.1 & 27.7 & 5.5 \\ 
Faucet  & 26.4 & 11.0 & 0.8 & 21.6 & 16.1 & 1.7 & 21.5 & 12.1 & 0.0 & 18.1 & 15.9 & 0.0 \\ 
\end{tabular}
\end{table*}
